Sum Rate Maximization for Movable Antenna-Aided Downlink RSMA Systems

Rate splitting multiple access (RSMA) is regarded as a crucial and powerful physical layer (PHY) paradigm for next-generation communication systems. Particularly, users employ successive interference cancellation (SIC) to decode part of the interference while treating the remainder as noise. However, conventional RSMA systems rely on fixed-position antenna arrays, limiting their ability to fully exploit spatial diversity. This constraint reduces beamforming gain and significantly impairs RSMA performance. To address this problem, we propose a movable antenna (MA)-aided RSMA scheme that allows the antennas at the base station (BS) to dynamically adjust their positions. Our objective is to maximize the system sum rate of common and private messages by jointly optimizing the MA positions, beamforming matrix, and common rate allocation. To tackle the formulated non-convex problem, we apply fractional programming (FP) and develop an efficient two-stage, coarse-to-fine-grained searching (CFGS) algorithm to obtain high-quality solutions. Numerical results demonstrate that, with optimized antenna adjustments, the MA-enabled system achieves substantial performance and reliability improvements in RSMA over fixed-position antenna setups.

==> Chapter/proposed_old.tex <==


\section{Proposed Solution}
To address this problem, we employ the fractional programming (FP) approach \cite{FPmethod,optimal_RSMA}. Auetaliary variables, including $\boldsymbol{\mu}=[\mu_1,\mu_2,...,\mu_{K}]^T$, $\boldsymbol{\eta}^c=[{\eta}^c_1,{\eta}^c_2,...,{\eta}^c_K]^T$, $\boldsymbol{\alpha}=[{\alpha}_1,{\alpha}_2,...,{\alpha}_K]^T$ and $\boldsymbol{\beta}=[{\beta}_1,{\beta}_2,...,{\beta}_K]^T$ are introduced to transform the objective function in (\text{P1}) and constraint (\ref{eq: common rate}) into equivalent convex forms as shown in (\ref{convexG}) and (\ref{update_eq: common rate}) respectively. 

Furthermore, we employ an AO algorithm to tackle the mutually coupled variables. Specifically, the beamforming matrix, splitting common rates, antenna positions, and auxiliary variables are updated in turn while the other parameters remain fixed until convergence is reached. (\text{P1}) can be divided into four sub-problems as follows.
\begin{equation*}
    (\text{SP.1}) \max_{\mathbf{F},\mathbf{r_c}}\hat{\mathcal{G}}(\mathbf{F},\mathbf{r_c}|\mathbf{x},\boldsymbol{\alpha},\boldsymbol{\beta},\boldsymbol{\mu},\boldsymbol{\eta})~\quad \\ \text{s.t.} \ \text{(\ref{eq: F}),(\ref{eq: positive rate}),(\ref{update_eq: common rate})},
\end{equation*}
\begin{equation*}
    (\text{SP.2}) \max_{\boldsymbol{\alpha},\boldsymbol{\mu}}\hat{\mathcal{G}}(\boldsymbol{\alpha},\boldsymbol{\mu}|\mathbf{x}, \mathbf{F},\mathbf{r_c},\boldsymbol{\beta},\boldsymbol{\eta})~\quad \\ \text{s.t.} \ \text{(\ref{update_eq: common rate})},
\end{equation*}
\begin{equation*}
    (\text{SP.3}) \max_{\boldsymbol{\beta},\boldsymbol{\eta}}\hat{\mathcal{G}}(\boldsymbol{\beta},\boldsymbol{\eta}|\mathbf{x}, \mathbf{F},\mathbf{r_c},\boldsymbol{\alpha},\boldsymbol{\mu})~\quad \\ \text{s.t.} \ \text{(\ref{update_eq: common rate})},
\end{equation*}
\begin{equation*}
    (\text{SP.4}) \max_{\mathbf{x}}\hat{\mathcal{G}}(\mathbf{x}|\mathbf{F},\mathbf{r_c},\boldsymbol{\alpha},\boldsymbol{\beta},\boldsymbol{\mu},\boldsymbol{\eta})~\quad \\ \text{s.t.} \ \text{(\ref{eq:x1}),(\ref{eq:x2}),(\ref{update_eq: common rate})}.
\end{equation*}

\subsubsection{Updating Beamforming Matrix and Allocating Common Rates}

[need more analysis]
By transforming 
Now, we can use the standard convex problem solvers such as
CVX to solve problem.

\subsubsection{Updating Auxiliary Variables for Quadratic Transform}
With other parameters fixed, we can update the auxiliary
variables. Since the objective function w.r.t. $\boldsymbol{\alpha}$ and the left side of (\ref{update_eq: common rate}) is concave w.r.t. $\boldsymbol{\beta}$. We can update them just by setting the patio derivative as zero i.e., $\frac{\partial \hat{\mathcal{G}}(\boldsymbol{\alpha},\boldsymbol{\mu}|\mathbf{x}, \mathbf{F},\mathbf{r_c},\boldsymbol{\beta},\boldsymbol{\eta})}{\partial \boldsymbol{\alpha}} = 0 $ and $\frac{\partial \hat{\mathcal{G}}(\boldsymbol{\alpha},\boldsymbol{\mu}|\mathbf{x}, \mathbf{F},\mathbf{r_c},\boldsymbol{\beta},\boldsymbol{\eta})}{\partial \boldsymbol{\mu}} = 0 $. Since there is no constraint for $\boldsymbol{\alpha}$ and updated $\boldsymbol{\beta}$ will not influence the correctness of (\ref{update_eq: common rate}). This gives

\begin{equation}
\alpha_k^*=\frac{|\mathbf{h}_k^H(x)\mathbf{f}_k|^2}{\sum\limits_{j=1, j \neq k}^{K} |\mathbf{h}_k^H(x)\mathbf{f}_j|^2 + \sigma_k^2},
\end{equation}

\begin{equation}
\mu_k^*=\frac{|\mathbf{h}_k^H(x)\mathbf{f}_c|^2}{\sum\limits_{j=1}^{K} |\mathbf{h}_k^H(x)\mathbf{f}_j|^2 + \sigma_k^2}.
\end{equation}



Similarly, the objective function is concave w.r.t. $\boldsymbol{\beta}$ and the left side of (\ref{update_eq: common rate}) is concave w.r.t. $\boldsymbol{\eta}$. By setting the patio derivative as zero, i.e., $\frac{\partial \hat{\mathcal{G}}(\boldsymbol{\alpha},\boldsymbol{\mu}|\mathbf{x}, \mathbf{F},\mathbf{r_c},\boldsymbol{\beta},\boldsymbol{\eta})}{\partial \boldsymbol{\alpha}} = 0 $ and $\frac{\partial \hat{\mathcal{G}}(\boldsymbol{\alpha},\boldsymbol{\mu}|\mathbf{x}, \mathbf{F},\mathbf{r_c},\boldsymbol{\beta},\boldsymbol{\eta})}{\partial \boldsymbol{\mu}} = 0 $. This gives

\begin{equation}
\beta_k^*=\frac{\sqrt{1+\alpha_k}\mathbf{h}_k^H(x)\mathbf{f}_k}{\sum\limits_{j=1}^{K} |\mathbf{h}_k^H(x)\mathbf{f}_j|^2 +\sigma_k^2},
\end{equation}

\begin{equation}
\eta_k^*=\frac{\sqrt{1+\mu_k}\mathbf{h}_k^H(x)\mathbf{f}_c}{\sum\limits_{j=1}^{K} |\mathbf{h}_k^H(x)\mathbf{f}_j|^2 + |\mathbf{h}_k^H(x)\mathbf{f}_c|^2+\sigma_k^2}.
\end{equation}




\subsubsection{Updating Antenna Positions}

Given the problem's non-convexity, obtaining optimal solutions is challenging. Following \cite{Peng2024JointAP}, we adopt a two-stage approach combining coarse and fine granularity methods to update antenna position.

CFGS is a two-stage searching algorithm. Firstly, find discrete samples separated by one lambda, and the point set is denoted as $S$. There is no need to conduct the whole optimization process to find the best initialization point positions. For each sample in $S$, we conduct one iteration of updating the beamforming matrix, splitting rates, and auxiliary variables. After that, we choose the sample with the best performance as the initialization points. 

Secondly, the gradient ascent method is adopted to adjust the antenna positions finely. The gradient of (\ref{convexG}) w.r.t. the $n^{th}$ antenna position $x_n$ can be derived as $\nabla \hat{\mathcal{G}}(x_n)=\sum\limits_{k=1}^{K}(\frac{\partial \hat{\mathcal{G}}_{1,k}(x_n)}{\partial x_n}-\frac{\partial \hat{\mathcal{G}}_{2,k}(x_n)}{\partial x_n})^T$, where $\frac{\partial \hat{\mathcal{G}}_{1,k}(x_n)}{\partial x_n}$ and $\frac{\partial \hat{\mathcal{G}}_{2,k}(x_n)}{\partial x_n}$ are shown in (\ref{F1_xn}) and (\ref{F2_xn}). This gives
\begin{equation}
    \mathbf{x}^{(s+1)}=\mathbf{x}^s+[\nabla \hat{\mathcal{G}}(x_1), \nabla \hat{\mathcal{G}}(x_2), \cdots, \nabla \hat{\mathcal{G}}(x_{N_T})]^T
\end{equation}

However conducting gradient ascent may make $x$ out of feasible region restricted by constraints (\ref{eq:x1}), (\ref{eq:x2}), (\ref{update_eq: common rate}). To ensure these constraints, we need to adjust the step size in each iteration \cite{MeiGA}. Define $R_s$ as the feasible region satisfying constraints (\ref{eq:x1}), (\ref{eq:x2}), (\ref{update_eq: common rate}). In the $(s+1)$-th iteration, if $x^{s+1}$ is not within the fesible set, i.e., $x^{s+1}\notin R_s$, the step size $\kappa$ is reduced to $\kappa /1.5$. This process will repeat until $x^{s+1}\in R_s$. The procedures are summarized in \textbf{Algorithm \ref{algoCFGS}}.

[!!! need a complexity analysis]





















\begin{figure*}[t]
    % \begin{align}
    %     &\max_{\mathbf{F}, \mathbf{r_c}, \mathbf{x}, \boldsymbol{\alpha},\boldsymbol{\beta}}\hat{\mathcal{G}}(\mathbf{F}, \mathbf{r_c}, \mathbf{x}, \boldsymbol{\alpha},\boldsymbol{\beta}) = \frac{1}{\log(2)}\sum\limits_{k=1}^{K}[\log(1+\alpha_k)-\alpha_k+2\sqrt{\alpha_k+1}\Re(\beta_k^*\mathbf{h}_k^H(x)\mathbf{f}_k)-|\beta_k|^2( \sum\limits_{j=1}^{K}|\mathbf{h}^H_k(x)\mathbf{f}_j|^2+\sigma_k^2)]+R_{c,k}.
    %     \label{convexG}
    % \end{align}


\begin{align}
\scalebox{0.91}{
$\hat{\mathcal{G}}(\mathbf{F}, \mathbf{r_c}, \mathbf{x}, \boldsymbol{\alpha},\boldsymbol{\beta}) = \underbrace{\frac{1}{\log(2)}\sum\limits_{k=1}^{K}[\log(1+\alpha_k)-\alpha_k]+R_{c,k}}_{\hat{\mathcal{G}}_0} + \underbrace{\frac{2}{\log(2)}\sum\limits_{k=1}^{K}\sqrt{\alpha_k+1}\Re\big(\beta_k^*\mathbf{h}_k^H(\mathbf{x})\mathbf{f}_k\big)}_{\hat{\mathcal{G}}_1} - \underbrace{\frac{1}{\log(2)}\sum\limits_{k=1}^{K}|\beta_k|^2( \sum\limits_{j=1}^{K}|\mathbf{h}^H_k(\mathbf{x})\mathbf{f}_j|^2+\sigma_k^2)}_{\hat{\mathcal{G}}_2}$},
\label{convexG}
\end{align}


% \begin{align}
%     \hat{\mathcal{G}_0}=\frac{1}{\log(2)}\sum\limits_{k=1}^{K}[\log(1+\alpha_k)-\alpha_k]+R_{c,k}
% \end{align}

% \begin{align}
% \hat{\mathcal{G}_1}=\frac{2}{\log(2)}\sqrt{\alpha_k+1}\Re(\beta_k^*\mathbf{h}_k^H(x)\mathbf{f}_k)
% \end{align}
% \begin{align}
%     \hat{\mathcal{G}_2}=-\frac{1}{\log(2)}|\beta_k|^2( \sum\limits_{j=1}^{K}|\mathbf{h}^H_k(x)\mathbf{f}_j|^2+\sigma_k^2)
% \end{align}


    \begin{align}
    \log(1+\mu_k)-\mu_k+2\sqrt{\mu_k+1}\Re(\eta_k^*\mathbf{h}_k^H(x)\mathbf{f}_c)-|\eta_k|^2( \sum\limits_{j=1}^{K}(|\mathbf{h}^H_k(x)\mathbf{f}_j|^2)+|\mathbf{h}^H_k(x)\mathbf{f}_c|^2+\sigma_k^2)\geq \log(2)\sum\limits_{j=1}^{K}R_{c,j},\forall k,
        \label{update_eq: common rate}
    \end{align}

    \begin{equation}
        \frac{\partial \hat{\mathcal{G}}_{1,k}(x_n)}{\partial x_n} = 2  \sqrt{\alpha_k+1}  \sqrt{\frac{\gamma_k}{L_p}}\operatorname{Re} \left\{ \sum_{l=1}^{L_p} j\rho_{k,l}\frac{2\pi}{d}\cos{\theta_{k,l}e^{j\frac{2\pi}{d}x_n\cos{\theta_{k,l}}}f_k^*\beta_k} \right\},
        \label{F1_xn}
    \end{equation}
    \begin{equation}
         \frac{\partial \hat{\mathcal{G}}_{2,k}(x_n)}{\partial x_n}=2|\beta_k|^2 \sqrt{\frac{\eta_k}{L_p} }j\frac{2 \pi}{\lambda} \operatorname{Re}\left\{\sum_{l=1}^{L_p}  \sum_{\substack{p=1}}^{L_p} \sum_{\substack{m=1}}^{N}  \cos \theta_{k,l} \rho_{k,l}^* \rho_{k,p} f_{j,n} f_{j,m}^* a_n^*(\theta_{k,l}) a_m(\theta_{k,p}) \right\}.
         \label{F2_xn}
    \end{equation}
    
\hrulefill
\end{figure*}

\begin{algorithm}[t]
    \renewcommand{\algorithmicrequire}{\textbf{Initialization:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
    \caption{Proposed CFGS algorithm for updating the antenna positions at Tx and Rx.}
     \label{algo2}
    \begin{algorithmic}[1]
        \REQUIRE Generate all the possible position alignments of transmit antenna as $\{ \bm{\zeta}_{x1}, \bm{\zeta}_{x2}, \cdots, \bm{\zeta}_{xq_{x}} \}$ from $\mathcal{S}_{X}$. And all the possible position alignments of receive antenna as $\{ \bm{\zeta}_{y1}, \bm{\zeta}_{y2}, \cdots, \bm{\zeta}_{yq_{y}} \}$ from $\mathcal{S}_{Y}$, set iteration index $l=1$.
        \FOR{$i=1,2,\cdots, q_{x}$}
            \FOR{$j=1,2,\cdots, q_{y}$}
            \STATE Let $\mathbf{x}=\bm{\zeta}_{xi}$ , $\mathbf{y}=\bm{\zeta}_{yj}$. 
            \STATE Converge $\mathbf{F}^{(ij)}$ and $\mathbf{w}^{(ij)}$ with \textbf{Algorithm \ref{algo1}}. 
            \STATE Compute $R_{ij}=\mathcal{G}(\mathbf{F}^{(ij)}, \mathbf{x}, \mathbf{y}, \mathbf{w}^{(ij)})$.
            \ENDFOR
        \ENDFOR
        \STATE Let $\mathbf{x}^{(0)}={\bm{\zeta}}_{xk}, \mathbf{y}^{(0)}={\bm{\zeta}}_{yt}, k,t=\arg\max R_{kt}$ .
        \REPEAT
            \STATE Converge $\mathbf{F}^{(l)}$ and $\mathbf{w}^{(l)}$ with \textbf{Algorithm \ref{algo1}}.
            \STATE Converge $\mathbf{x}^{(l)}$ and $\mathbf{y}^{(l)}$ as (\ref{x_update}) and (\ref{y_update}). 
            \STATE Adjust $\mathbf{x}^{(l)}$ and $\mathbf{y}^{(l)}$ as (\ref{eq:antenna projection}).
            \STATE Update iteration index $l=l+1$.
        \UNTIL{the value of objective function converge.}
        \ENSURE $\mathbf{x}^{(l-1)}$ and $\mathbf{y}^{(l-1)}$ 
    \end{algorithmic}
    \label{algoCFGS}
\end{algorithm}

\section{Numerical Results}
In addition to our proposed FP-based and CFGS-based algorithm with MAs \textbf{(FP-CFGS, MAs)}, two schemes are compared: FP-based fixed position antenna \textbf{(FP, FPA)} and FP-based with direct gradient ascent movable antennas \textbf{(FP-DGA, MAs)}. In the former scheme, the antenna spacing is assumed to be fixed as $\lambda/2$. In contrast, the antenna positions are assumed to be uniformly distributed initially, and finely antenna adjustments are conducted directly using gradient ascent in the latter scheme. The initial beamforming matrix configuration is based on the approach in \cite{SR_RSMA}. Here, the private beamforming vectors are designed using maximum ratio transmission (MRT), while the common beamforming vector is constructed based on the dominant left singular vector of the channel matrix H, where $H=[h_1,\cdots,h_K]$.


We consider path number $L_p = 8$ for $K = 4$ users, respectively. Users are randomly positioned around the BS within the angle range $[0,\pi]$. User-BS distances are randomly distributed within $[20\,\text{m}, 100\,\text{m}]$. The channel gain follows the standard complex Gaussian distribution, i.e., $\alpha_{s},\alpha_{c},\rho_{k,l} \sim \mathcal{C}\mathcal{N}(0,1)$. According to the simulation setup of \cite{PowerNOMA}, given a carrier frequency of 5 GHz, the wavelength is $\lambda=0.06$ m. The elements of PRV follow the CSCG distribution, i.e., $g_k \sim  \mathcal{CN}\left(0, \frac{C_{k}^2}{L}\right)$. The term $C_{k}^2=C_0D_k^{-\tau}$, where $C_0=\frac{\lambda}{4\pi^2}$ is the expected average channel power gain at the reference distance of 1 m and the path-loss exponent $\tau= 2.8$ is the path-loss exponent, respectively. The received noise power is $-90$ dBm. Additionally, without loss of generality, the feasible lower bound for MAs $X_{\min}$ is set to 0, and $D_0$ is set as $\frac{\lambda}{2}$, respectively. 


Fig. \ref{fig:power_comparison} illustrates the ISAC performance across varying transmit power levels and different antenna configurations. The transmit power ranges from 20 dBm to 40 dBm, with three sets of antenna number configurations used in the simulation: $\{8,4\}$, $\{10,4\}$, and $\{8,6\}$ for transmit and receive antennas, respectively.
The result shows that the objective function grows with increasing transmit power and the number of antennas. When transmit power $P_0$ = 40 dBm, 8 transmit antennas and 4 receive antennas are used. The objective function increases by 10.9\% with GA-MA compared to FPA, and a 27.79\% increment when CFGS-MA is used compared to FPA.
Furthermore, for all three sets of antenna number in the simulation, CFGS-MA shows a better performance than GA-MA and FPA. 

Fig. \ref{fig:range_comparison} shows the ISAC performance with different movable range of transmit and receive antennas. The movable range of the transmit antennas varies from 8 $\lambda$ to 14 $\lambda$,  while the receive antennas are tested with three different movable ranges: 6 $\lambda$, 8 $\lambda$, and 10 $\lambda$. The results show that with GA-MA, performance improvement is small, as it only achieves a local optimum near the initial position, limiting the benefit of a larger movable range. In contrast, the proposed CFGS-MA significantly enhances performance, with an 11.47\% increase in the objective function as the transmit movable range expands from 8 $\lambda$ to 14 $\lambda$ with the receive movable range is 8 $\lambda$. Additionally, there is a 1.46\% increase as the movable range of receive antennas varies from 6 $\lambda$ to 10 $\lambda$ while maintaining transmit antennas' movable range at 12 $\lambda$. These results demonstrate that CFGS-MA effective utilization of the available range.







\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{figs/fig1.png}
    \caption{ISAC performance with different transmit power, $X_{\max}=12\lambda$, $Y_{\max}=8\lambda$, $\varpi_s=0.5$ and $\varpi_c=0.5$, $r_{0}=20\lambda$.}
   \vspace{-0.2cm}
    \label{fig:power_comparison}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{figs/fig2.png}
    \caption{ISAC performance with different antenna movable range, $P_0=30$ dBm, $N_T=8$, $N_R=4$, $\varpi_s=0.5$ and $\varpi_c=0.5$, $r_{0}=20\lambda$.}
    \vspace{-0.3cm}
    \label{fig:range_comparison}
\end{figure}

\section{Conclusion}
In conclusion, this paper presents a movable antenna (MA)-enabled downlink 1-layer rate splitting multiple access (RSMA) system designed to fully exploit spatial freedom by allowing dynamic adjustments of antenna positions at the BS. By jointly optimizing MA positions, beamforming matrix, and common rate allocation, we aim to maximize the system's sum throughput, including both common and private messages. Although this approach leads to a challenging non-convex optimization problem, we address it by employing FP and a coarse-to-fine-grained searching algorithm to derive suboptimal solutions. Simulation results validate the effectiveness of the proposed scheme, demonstrating that the MAs-enabled system substantially improves the performance and reliability of RSMA compared to conventional fixed-position antenna designs when using our algorithm. 








==> formula-part.tex <==
% \section{System model}

% \subsection{$H_{SI}$ model}

% \textbf{Near field LOS model:}
% \begin{equation}
% \mathbf{H}(n_1, n_2) = \frac{1}{r_{n_1, n_2}} e^{-j \frac{2\pi}{\lambda} r_{n_1, n_2}},
% \end{equation}


% \begin{equation}
% \begin{split}
% r(x_i,y_j) = & \sqrt{r^2 + x_i^2 + y_j^2 + 2ry_j\sin(\theta-\phi) \\
% & - 2rx_i\sin\theta - 2x_iy_j\cos\phi}
% \end{split}
-% \end{equation}




% \begin{equation}
% \mathbf{R(x,y)} = \begin{bmatrix}
% r(x_1,y_1) & \cdots  & r(x_1,y_{N_R}) \\
% \vdots & \ddots  &\vdots \\
% r(x_{N_T},1) & \cdots  & r(x_{N_T},y_{N_R})
% \end{bmatrix}
% \end{equation}

% \begin{equation}
% \begin{split}
% H_{SI} = & \mathbf{H}_{LOS}(R(\mathbf{x},\mathbf{y}),\theta,\phi) \\
% = & \begin{bmatrix}
% H(x_1,y_1) & \cdots  & H(x_1,N_R) \\
% \vdots & \ddots  & \vdots \\
% H(x_{N_T},y_1) & \cdots  & H(x_{N_T},y_{N_R})
% \end{bmatrix}\in \mathbb{C}^{N_T \times N_R}
% \end{split}
% \end{equation}


% After channel estimation to obtain $\theta,\phi$, $H_{SI}=V(\mathbf{x,y})$.

% \subsection{Communication part model}
% \begin{equation}
% \mathbf{h}_k(\mathbf{x}) = \sqrt{\frac{N_t}{L_p}} \sum\limits_{l=1}^{L_p} \rho_{k,l} \mathbf{a}_{k,l}(\mathbf{x})\in \mathbb{C}^{N_T \times 1}
% \end{equation}

% Steering vector:
% \begin{equation}
% \small
% \mathbf{a}_{k,l}(\mathbf{x}) = \begin{bmatrix} 1 & e^{j\frac{2\pi }{\lambda} x_1\cos(\theta)}  & \cdots & e^{j\frac{2\pi }{\lambda} x_{N_T}\cos(\theta)} \end{bmatrix}^T\in \mathbb{C}^{N_T \times 1}
% \label{steering_vector}
% \end{equation}

% Precoding matrix:
% \begin{equation}
% \mathbf{F}=[\mathbf{f_1},\mathbf{f_2},...,\mathbf{f_K}]\in \mathbb{C}^{N_T \times K}
% \end{equation}
% The power for each antenna can be defined as:

% \begin{equation}
% \mathbf{\bar{f}}(n)=[f_1(n),...,f_K(n)]^T\in \mathbb{C}^{K \times 1}
% \end{equation}

% \begin{equation}
% \hat{\mathbf{f}}=[\|\mathbf{\bar{f}}(1)\|_2, ...,\|\mathbf{\bar{f}}(N_T)\|_2]^T\in \mathbb{C}^{N_T \times 1}
% \end{equation}

% For K users, signals are $\mathbf{s}=[s_1,s_2,...,s_K]^T\in \mathbb{C}^{K \times 1}$, used both for sensing and communication:
% \begin{equation}
% y_k = \mathbf{h}_k^H(x)\mathbf{f_k}s_k + \mathbf{h}_k^H\sum\limits_{j=1, j\neq k}^{K} \mathbf{f}_j s_j + n_k \in\mathbb{C}
% \end{equation}

% \begin{equation}
% R_k=\log_2(1+\text{SINR}_k)
% \end{equation}

% \begin{equation}
% \text{SINR}_k = \frac{|\mathbf{h}_k^H(x)\mathbf{f}_k|^2}{\sum\limits_{j=1, j \neq k}^{K} |\mathbf{h}_k^H(x)\mathbf{f}_j|^2 + \sigma_k^2}
% \end{equation}

% \subsection{Sensing part model (with no clutters)}
% Current transmitted signals are still $\mathbf{s}$.
% Received signal before received beamforming:
% \begin{equation}
% \mathbf{y_{0s}} = \alpha_s \mathbf{b}_s(\mathbf{y}) \mathbf{a}_s^H(\mathbf{x}) \mathbf{F} \mathbf{s}  + \mathbf{H_{SI}} 
%    (\mathbf{x},\mathbf{y})\mathbf{F} \mathbf{s}+\mathbf{n_s}\in \mathbb{C}^{N_R \times 1}
% \end{equation}

% Received signal after received beamforming:
% \begin{align}
% y_{1s} &= \mathbf{w_r}^H  \mathbf{y_{0s}} \notag \\
% &= \alpha_s \mathbf{w_r}^H \mathbf{b}_s(\mathbf{y}) \mathbf{a}_s^H(\mathbf{x}) \mathbf{F} \mathbf{s} \notag \\
% &\quad + \mathbf{w_r}^H \mathbf{H_{SI}}(\mathbf{x}, \mathbf{y}) \mathbf{F} \mathbf{s} \notag \\
% &\quad + \mathbf{w_r}^H \mathbf{n_s} 
% \end{align}

% \begin{equation}
% \text{SINR}_s = \frac{|\alpha_s\mathbf{w_r}^H \mathbf{b}_s(\mathbf{y})\mathbf{a}_s^H(\mathbf{x}) \mathbf{F}|^2}{|\mathbf{w_r}^H H_{SI}(\mathbf{x},\mathbf{y})\mathbf{F}|^2+ \sigma_s^2}
% \end{equation}

% \begin{equation}
% R_s = \log_2(1 + \text{SINR}_s)
% \end{equation}

% $\left\|\mathbf{w_r}\right\|^2=1,\mathbf{a}_s(\mathbf{x})\in \mathbb{C}^{N_T \times 1},\mathbf{b}_s(\mathbf{y})\in \mathbb{C}^{N_R \times 1} $ are steering vectors for transmitter and receiver respectively. (Their forms are similar to Formula.\ref{steering_vector})
% \clearpage
% \newpage

% \section{Optimization problem}
% \begin{equation}
% \text{(P1)} \quad \max_{\mathbf{F}, \mathbf{x},\mathbf{y},\mathbf{w_r}} \mathcal{G}(\mathbf{F}, \mathbf{x},\mathbf{y},\mathbf{w_r}) = \varpi_c \sum\limits_{k=1}^{K} R_k + \varpi_s R_s,
% \label{optimizationproblem}
% \end{equation}

% \begin{equation}
% \text{s.t.} \quad \text{Tr}(\mathbf{F}^H \mathbf{F}) \leq P_0, E{\{ss^H\}}=\mathbf{I},\left\|\mathbf{w_r}\right\|^2=1
% \end{equation}

% \begin{equation}
% P_{PA} + P_A \|\hat{\mathbf{f}}\|_0 \leq P_{tot}
% \end{equation}

% \begin{equation}
% \mathbf{x} \in \mathcal{A}, \mathbf{y} \in \mathcal{B}, |x_a-x_b|\geq D_0,|y_c-y_d|\geq D_0
% \end{equation}


% The problem(\ref{optimizationproblem}) is equivalent to P2 with Lagrangian dual transform (to be proofed)

% \begin{align}
%     \text{(P2)} &\quad \mathcal{G}_d(\mathbf{F}, \mathbf{x},\mathbf{y},\mathbf{w_r},\mu) =  \varpi_c \sum\limits_{k=1}^{K} log_2(1+\mu_k) + \varpi_s log_2(1+\mu_{K+1}) - \varpi_c \sum\limits_{k=1}^{K} \mu_k - \varpi_s \mu_{K+1} \notag \\ 
%     & + \varpi_c\sum\limits_{k=1}^{K}\left(\frac{(1+\mu_k)|\mathbf{h}_k^H(x)\mathbf{f}_k|^2}{\sum\limits_{j=1}^{K} |\mathbf{h}_k^H(x)\mathbf{f}_j|^2 + \sigma_k^2} \right) \\
%     &+\varpi_s \frac{|\alpha_s\mathbf{w_r}^H \mathbf{b}_s(\mathbf{y})\mathbf{a}_s^H(\mathbf{x}) \mathbf{F}|^2}{\sum_{c=1}^C|\alpha_c\mathbf{w_r}^H \mathbf{b}_c(\mathbf{y})\mathbf{a}_c^H(\mathbf{x}) \mathbf{F}|^2 
%     +|\alpha_s\mathbf{w_r}^H \mathbf{b}_s(\mathbf{y})\mathbf{a}_s^H(\mathbf{x}) \mathbf{F}|^2 
%     + |\mathbf{w_r}^H H_{SI}(\mathbf{x},\mathbf{y})\mathbf{F}|^2+ ||w_r||^2\mathbf{\sigma_s}^2}  \notag\\
%     & = \varpi_c \sum\limits_{k=1}^{K} log_2(1+\mu_k) + \varpi_s log_2(1+\mu_{K+1}) - \varpi_c \sum\limits_{k=1}^{K} \mu_k - \varpi_s \mu_{K+1} \notag  \\
%     & +\varpi_c\sum_{k=1}^{K}\left(2\sqrt{1+\mu_k}Re\{\xi^c_k h_k^H(x)f_k(x)\}-|\xi^c_k|^2\left(\sum_{j=1}^K|h_k^H(x)f_j|^2+\sigma_k^2\right)\right) \notag \\
%     & + \varpi_s [ 2\sqrt{1+\mu_{K+1}}Re\{\alpha_s w_r^H b_s(y)a_s^H(x)F\xi^s\} \notag \\
%     &-||\mathbf{\xi}^s||^2\left(\sum_{c=1}^C||\alpha_c w_r^H b_c(y) a_c^H(x)F||^2+||w_r^H H_{SI}^H(x,y)F||^2+||\alpha_s w_r^H b_s(y)a_s^H(x)F||^2+||w_r||^2 \mathbf{\sigma}_s^2\right)]
% \end{align}

% in which,
% \begin{align*}
%     \Lambda_k &= \varpi_c HH^H  + \varpi_s ||\xi^s||^2 \Bigg[
%     \sum_{c=1}^C |\alpha_c|^2 \left(w_r^H b_c(y) a_c^H(x) \right)^H \left(w_r^H b_c(y) a_c^H(x) \right) \\
%     &\quad + |\alpha_s|^2 \left(w_r^H b_s(y) a_s^H(x) \right)^H \left(w_r^H b_s(y) a_s^H(x) \right)  + \left(w_r^H H_{SI}^H(x,y)\right)^H \left(w_r^H H_{SI}^H(x,y)\right) 
%     \Bigg]
% \end{align*}

% \begin{equation*}
% \phi_k=\varpi_c\sqrt{1+\mu_k}\xi^{c(t)*}h_k(x^{(t)})+\varpi_s\sqrt{1+\mu_{K+1}} \alpha_s^{*}\xi^{s(t)*}_k a_s(x^{(t)})b^H_s(y) w_r
% \end{equation*}

% \begin{equation}
%     B=\varpi_c\sum^K_{k=1}ln(1+\mu_k)+\varpi_s ln(1+\mu_{K+1})-\varpi_c\sum_{k+1}\mu_k-\varpi_s\mu_{K+1}-\varpi_c\sum^K|\xi^c_k|^2\sigma_k^2-\varpi_s||\xi^2||...
% \end{equation}
% and with quadratic transform, the sum-of-ratio term can be transformed into ,and 
% \clearpage
% \newpage

% \begin{align}
% \nabla L_{w_r} = \varpi_s & \left\{ \sqrt{\mu_{K+1}+1} \alpha_s^* b^*_s(y) a_s(x) F^* \xi^{s*} \right. \nonumber \\
% & - ||\xi^s||^2 \left( \sum_{c=1}^C |\alpha_c|^2 \left( b_c(y) a_c^H(x) F \right)^* \left( b_c(y) a_c^H(x) F \right)^T w_r^* \right. \nonumber \\
% & + (H_{SI}^H(x,y) F)^* (H_{SI}^H(x,y) F)^T w_r^* \nonumber \\
% & + |\alpha_s|^2 (b_s(y) a_s^H(x) F)^* (b_s(y) a_s^H(x) F)^T w_r^* \nonumber \\
% & \left. \left. + w_r^* \mathbf{\sigma}_s^2 \right) \right\}
% \end{align}

% \begin{align}
%     \Psi&=||\xi^s||^2\left\{\sum|\alpha_c|^2\left(b_c(y)a_c^H(x)F\right)\left(b_c(y)a_c^H(x)F\right)^H+\left(H_{SI}^H(x,y)F\right)\left(H_{SI}^H(x,y)F\right)^H \right. \nonumber\\
%     & \left. +|\alpha_s|^2\left(b_s(y)a_s^H(x)F\right)\left(b_s(y)a_s^H(x)F\right)^H+\sigma_x^2I\right\}
% \end{align}

% \begin{equation}
%        \Delta=\sqrt{1+\mu_{K+1}}\alpha_sb_s(y)a_s^H(x)F\xi^s
% \end{equation}

% \begin{equation}
%     w_r=\left\{\left\{\Psi\right\}^{-1}\right\}^*
%     \left\{\Delta\right\}\nonumber \\
% \end{equation}


% \begin{align}
%     &w_r=\left\{\left\{||\xi^s||^2\left(\sum|\alpha_c|^2\left(b_c(y)a_c^H(x)F\right)\left(b_c(y)a_c^H(x)F\right)^H+\left(H_{SI}^H(x,y)F\right)\left(H_{SI}^H(x,y)F\right)^H\nonumber \right.\right.\right.\\
%     & \left.\left.\left.+|\alpha_s|^2\left(b_s(y)a_s^H(x)F\right)\left(b_s(y)a_s^H(x)F\right)^H+\sigma_x^2I\right)\right\}^{-1}\right\}^*
%     \left\{\sqrt{1+\mu_{K+1}}\alpha_sb_s(y)a_s^H(x)F\xi^s\right\}\nonumber \\
% \end{align}

% \begin{align}
%     &\mathbf{\xi}^{s(t+1)}=\frac{\sqrt{1+\mu_{K+1}}\alpha_s^* w_r^Tb_s^*(y)a_s^T(x)F^*}{I_M+||w_r||^2 \mathbf{\sigma}_s^2} \nonumber\\
% \end{align}

% \begin{equation}
%     I_M=\sum_{c=1}^C||\alpha_c w_r^H b_c(y) a_c^H(x)F||^2+||w_r^H H_{SI}^H(x,y)F||^2+||\alpha_s w_r^H b_s(y)a_s^H(x)F||^2
% \end{equation}

% \begin{equation}
%     I_M=\sum_{c=1}^C||\alpha_c w_r^H b_c(y) a_c^H(x)F||^2+||w_r^H H_{SI}^H(x,y)F||^2+||\alpha_s w_r^H b_s(y)a_s^H(x)F||^2
% \end{equation}

% % \begin{equation}
% %     \beta=\left[ \frac{\sqrt{G_l}\lambda}{4 \pi d_{u,k}} \right]^2
% % \end{equation}

% \begin{equation}
%     c^2_{kj}=\beta_0d_{kj}^{-\alpha_0}
% \end{equation}
% \begin{equation}
%     \alpha \sim \mathcal{CN}\left(0, \frac{c^2_{kj}}{L_p}\right)
% \end{equation}




% \clearpage
% \newpage

% \begin{table}[h]
% \centering
% \caption{Parameters of the FD ISAC system} % 表格标题
% \label{table:1}
% \begin{tabular}{ccc}
% \toprule
% Parameter & Notation & Value \\
% \midrule
% user clutter angle& &$[0,\pi]$\\
% Carrier frequency &$f_c$& 2.4 GHz\\
% Wavelength & $\lambda$ & 0.125 m\\
% Distance between user and BS & $d_{u,b}$ &  [50m,80m]\\
% Distance between object and BS & $d_{u,b}$ &  [10m,20m]\\
% Distance between RX and TX & $d_{TX,RX}$ & 1.25 m\\
%   &$\beta_0$& -40\\
% Pathloss exponent  &$\alpha_0$&2.8\\
% Transmit power  &$P_t$&15 dBm\\
% Receive noise power  &$\sigma_r^2$&-80 dBm\\

% \bottomrule
% \end{tabular}
% \end{table}


% \section{Remaining Problems}
% Unsolved:
% \begin{enumerate}[label=\arabic*)]
%     \item needs one graph for the system model and one graph for the near-field model
%     \item need one paper use only use the beamforming method instead of physical isolation in propagation domain
%     \item D1 how to define?
%     \item Shall we add SI channel K (match to the real scenario)?
% \end{enumerate}
% Solved:
% \begin{enumerate}[label=\arabic*)]
%     \item any constraints for receiving beamforming matrix
%     \item has not added the antenna selection condition
%     \item do not add the receive beamforming matrix(be careful about the dimension)
% \end{enumerate}
